Non-linear Phenomenology of Disformally Coupled Quintessence

The Quintessence model is one of the simplest and better known alternatives to Einstein's theory for gravity. The properties of the solutions have been studied in great detail in the background, linear and non-linear contexts in cosmology. Here we discuss new phenomenology that is induced by adding disformal terms to the interactions. Among other results, we show analytically and using cosmological simulations ran with the code \texttt{Isis} that the model posses a mechanism through which is it possible to obtain repulsive fifth forces, which are opposite to gravity. Although the equations are very complex, we also find that most of the new phenomenology can be explained by studying background quantities. We used our simulation data to test approximate relations that exist between the metric and scalar field perturbations as well as between the fifth force and gravity. Excellent agreement was found between exact and approximated solutions, which opens the way for running disformal gravity cosmological simulations using simply a Newtonian solver. These results could not only help us to find new ways of testing gravity, but also provide new motivations for building alternative models.

==> table_model.tex <==
%============================================================================
    \hline
    \emp{0.3}
    
    \emp
    &
    \bmp{0.4}  
        {
          \begin{flalign*}
            
          \end{flalign*}
        }
     \emp
     \bmp{0.4}
         { \begin{flalign*}
             
         \end{flalign*} }
      \emp
      \\
      & \bmp{0.6}
      
      \emp


